Set Learning for Accurate and Calibrated Models

Model overconfidence and poor calibration are common in machine learning and difficult to account for when applying standard empirical risk minimization. In this work, we propose a novel method to alleviate these problems that we call odd-$k$-out learning (OKO), which minimizes the cross-entropy error for sets rather than for single examples. This naturally allows the model to capture correlations across data examples and achieves both better accuracy and calibration, especially in limited training data and class-imbalanced regimes. Perhaps surprisingly, OKO often yields better calibration even when training with hard labels and dropping any additional calibration parameter tuning, such as temperature scaling. We demonstrate this in extensive experimental analyses and provide a mathematical theory to interpret our findings. We emphasize that OKO is a general framework that can be easily adapted to many settings and a trained model can be applied to single examples at inference time, without significant run-time overhead or architecture changes.

==> checklist.tex <==
\section*{Checklist}
\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{See \S~\ref{sec:conclusion}.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNA{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{} %TODO: is this true?
        \item Did you include complete proofs of all theoretical results?
    \answerYes{}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)? \answerYes{See \url{https://github.com/LukasMut/VICE} for our codebase. See \url{https://osf.io/jum2f/} and \url{https://things-initiative.org/} for data.}
    
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{See \S~\ref{sec:data}, \S~\ref{sec:experimental_setup} and Appendix~\ref{app:experimental_details}.}
    \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{See Figure~\ref{fig:data_effiency} and Table~\ref{tab:reliability}.}
    \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{See Appendix~\ref{app:experimental_details}}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerYes{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{See \url{https://github.com/LukasMut/OKO}.}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerYes{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerYes{See Appendix~\ref{app:dataset_details}.}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
    
%TODO: Write a sentence about the crowdsourced data you use
\end{enumerate}

We re-used crowdsourced data collected by various collaborators, and attribute it to them in the main paper. Even though we did not collect these data ourselves, we provide a summary of the information asked for in 5. in Appendix~\ref{app:dataset_details}, as well as a short description of the task and stimuli in Section~\ref{method:triplet_task}.

\end{enumerate}


==> holding.tex <==
\section{Working Zone: OKO and Calibration}


%Rare classes make it difficult for calibration in practice, that is the predicted probabilities match the true probabilities of an event occurring, essential for making reliable decisions based on the model's predictions. Specifically, if $f : \gX \to [0, 1]$ is a probabilistic model for binary labels, we want $\E[y | f(x) = v] = v$. For multi-class labels, this generalizes for each class such that for predicted probability vector $p \in [0,1]^C$, $\E[\ve_y | f(x) = p] = p$. 



\iffalse


As a toy example, consider two classes $C_1$, $C_2$ with only 1 input feature $x$. 
Data Assumptions
Let’s say that our data is split into three clusters: 

\begin{enumerate}
\item When $x$ is around 1, all $n_1$ data points have label $y_1 = \ve_1$
\item When $x$ is around -1, all $n_2$ data points have label $y_2 = \ve_2$ 
\item When $x$ is around 0, $n_{01}$ datapoints have label $\ve_1$ and $n_{0,2}$ have label $\ve_2$ and $n_0 = n_{01} + n_{02}$
\end{enumerate}

Since the clusters at the edges of $x$ are clearly separable, we know that $f(1) = \ve_1$ and $f(-1) = \ve_2$. However, in the middle, since our predictor $f(x)$ is smooth, we generally will want $f(x) = (p_1, p_2)$, where $p_i = n_{0i}/n_0$. 




The main interest optimization is to find the best value of $P(0)$ and so if we let $s_i = n_{0i}/{m_i}$ be the proportion of the class has $x_i = 0$, we can rewrite the loss as $s_1 \ve_1^\top \log (P(0)) + s_2 \ve_1^\top \log (P(0))$.  Then note that the optimal F would satisfy:

\begin{itemize}
    \item $P(1) = \ve_1$
    \item $P(-1) = \ve_2$
    \item $P(0) =  c_0 * <s_1, s_2>$
\end{itemize}

for some normalizing constants $c_0$ since minimizing the cross entropy loss would result in these proportions. Note that $F(1), F(-1), F(0)$ are all optimized individually.

However, note that in set learning, there are interdependencies on the values of $F$ and the  resulting probabilities would not be some extreme. Specifically,


\begin{align*}
    \gL (\theta) &\propto \frac{1}{m_1^2m_2}  \sum_{x_1, x_2 \in C_1, x_3 \in C_2} -\ve_1^\top \log(\softmax( F(\{x_1, x_2, x_3\}))) \\
    &\hspace{.5in} + \frac{1}{m_1m_2^2} \sum_{x_1, x_2 \in C_2, x_3 \in C_1} -\ve_2^\top \log(\softmax( F(\{x_1, x_2, x_3\}))) \\
\end{align*}

Let us try to decompose the first sum. Note that we have the following situation of the different types of sets we could have:

\begin{itemize}
    \item $x_1, x_2 = 1$ and $x_3 = -1$ \hspace{.2in} (mass = $(1-s_1)^2(1-s_2)$)
    \item $x_1, x_2 = 1$ and $x_3 = 0$  \hspace{.2in} (mass = $(1-s_1)^2s_2$)
    \item One of $x_1, x_2$ is 1 and $x_3 = -1$ \hspace{.2in} (mass = $2s_1(1-s_1)(1-s_2)$)
    \item One of $x_1, x_2$ is 1 and $x_3 = 0$ \hspace{.2in} (mass = $2s_1(1-s_1)s_2$)
    \item $x_1, x_2 = 0$ and $x_3 = -1$ \hspace{.2in} (mass = $s_1^2(1-s_2)$)
    \item $x_1, x_2 = 0$  and $x_3 = 0$ \hspace{.2in} (mass = $s_1^2s_2$)
\end{itemize}

Note that mass is the proportion of the total $m_1^2m_2$ sets that have the specific type. Let's assume that $s_1, s_2$ are small since the models usually have enough capacity to differentiate between most datapoints, resulting in relatively large accuracy. Therefore, we may approximate $1-s_i \approx 1$ and notice that the majority of the loss is dominated by:

$$\gL (\theta) \propto  (1-s_1)^2(1-s_2) \ve_1^\top(\log(\softmax(2F(1) + F(-1)))) + (1-s_2)^2(1-s_1) \ve_2^\top(\log(\softmax(F(1) + 2F(-1))))$$

This implies that the optimal $F$ (and corresponding $P$) at $1, -1$ will satisfy $P(1) \approx \ve_1$ and $P(-1) \approx \ve_2$, as is in the standard vanilla setting. 

However, to see the setting of $F(0)$, we focus the linear terms of the loss are now:

$$ s_2\ve_1^\top\log(\softmax(2F(1) + F(0))) + s_1\ve_2^\top\log(\softmax(2F(-1) + F(0)))$$
$$+s_1\ve_1^\top\log(\softmax(F(\{1,0,-1\}))) + s_2\ve_2^\top\log(\softmax(F(\{1,0,-1\})))$$


Note that the first two terms are relatively small since $F(1), F(-1)$ will favor classes $C_1, C_2$ respectively, as mentioned above. Therefore, we see that if we assume that the optimal value of $F(\{1, 0, -1\})$ show lead to predictions that are in fact: $$P(\{1, 0, -1\}) \propto < s_1, s_2>$$ 

In terms of $F$, this means that $\Delta F(\{1, 0, -1\}) = \log(s_2) - \log(s_1)$, where $\Delta F (x) = (\ve_2 - \ve_1)^\top F (x) $ Now, consider WLOG the case when $s_1 \leq s_2$ and note that now we have two quadratic terms in the loss, specifically together we have the one that is going the wrong way is:

$$ s_1^2 \ve_1^\top \log(\softmax(2F(0) + F(-1))) + s_1 s_2 \ve_1^\top \log(\softmax( 2F(0) + F(1)) $$ 
$$ \, + s_1 s_2 \ve_2^\top \log (\softmax(2F(0) + F(-1))) + s_2^2 \ve_2^\top \log(\softmax(2F(0) + F(1)))$$

To minimize this, we want $2\Delta F(0) + \Delta F(1) = \log(s_2^2) - \log(s_1s_2) = \log(s_2) - \log(s_1)$ and similarly, $2\Delta F(0) + \Delta F(-1) = \log(s_2) - \log(s_1)$.  to be as large as possible. However, since $\Delta F(-1) + \Delta F(0) + \Delta F(1) = \log(s_2) - \log(s_1)$, this implies that $\Delta F(0) = \Delta F(1) = \Delta F(-1)$. 




Similarly, we 
Since $F(0) = <l_1, l_2>$, where $l_1 \leq l_2$ by assumption, we know that the quadratic term is dominated by the second term: $s_2^2 \ve_2^\top \log((\softmax(2F(0) + F(1))))$. However, this term must enforces scaling similarity between $F(0)$ and $F(1)$. Therefore the scale of $F(0), F(1), F(-1)$ are no longer independent.


Observations

Note: Consider a small bias. But note that if $s_1, s_2$ are small, then we want $<c_1 + c_0 l_1, c_2>$  to be biased towards label 1 and vice versa for label 2. Therefore, we want to set $c_0$ relatively large and $l_1, l_2$ to be relatively equal…if fact the optimal-ish is when we can set logits at cluster 0 to be around $<½, ½>$. This will boost accuracy on the underrepresented class (as defined by the argmax). Intuitively, this is because the loss includes a label from the well-separated clusters with probability $1 - s_1^2$ and so, it does not need to focus on the non-separated clusters at x = 0 to differentiate proportionally (this should improve calibration and accuracy in ambiguous regions, esp. for underrep classes).


Perhaps this is very similar to inducing more label entropy (i.e. adding label noise), especially in regions of disagreement. Actually this loss objective may be slightly biased towards uncertainty (higher entropy predictions).
\fi

Generally, the data distribution is for a noisy dataset, which we model using a toy but important example that illustrates why OKO is able to produce higher entropy predictions especially in the high noise regime, as that would be desired (and this helps theoretically justify the higher entropy behavior that is empirically observed by our experiments).
Consider any dataset $\mathcal{D}$, which has datapoints $(x_i, y_i)$ such that none of the feature vectors $x_i$ overlap and for sake of illustration, we let the classes $y_i$ to be separable. In $\mathcal{D}$, we expect any classifier to have full accuracy with high confidence. 

Now we construct our noisy dataset $\mathcal{D}'$ by appending to it the noisy examples $\{(x , y_{i})\}_{i=1}^k$, where $x$ is a shared feature vector across all of the $y_{i}$ labels where $x$-to-$y$ is a one-to-many-mapping (i.e., the input $x$ is associated with different labels). Since the labels are noisy there this creates high uncertainty around the input $x$. However, with sufficiently many of such noisy labels, the classifier should also start to be less confident about its predictions on $\mathcal{D}$, as the vast majority of examples in each class become noisy. 


\begin{lemma}
\label{lem:regularization}
Let $\mathcal{D}$ be any dataset and construct $\mathcal{D}'$ by appending $(x, y_i)$ to $\mathcal{D}$ for some shared feature vector $x$ such that for all classes $C_i$, exactly $1-\epsilon$ fraction of the datapoints in $C_i$ has feature $x$. Furthermore, assume that in our domain of $\theta \in \Theta$, $-\log(\softmax(f_\theta(\gS))) \leq B$ is bounded element-wise for any set $\gS$. Let $\theta^{\star}$ be parameters such that $H(f_{\theta^\star}(x')) = \log(|C|)$ has maximal entropy for all features $x' \in \mathcal{D}'$. 

Then, $\theta^\star$ is an approximate minimizer of the OKO loss $\gL$:

$$\gL(\theta^\star) \leq \min_{\theta \in \Theta} \gL(\theta) + O(B\epsilon^2)$$

Specifically, this implies that the expected excess loss conditioned on sets with non-shared features $x' \neq x$ is bounded by $O(B\epsilon)$. 
\end{lemma}

\begin{proof}[Proof of Lemma~\ref{lem:regularization}]
As we did previously, we denote $f_\theta(\gS_x) = \sum_{s \in \gS_x} f_\theta(s) = \sum_{y_i \in \gS_y} F_{y_i}$, where for the lowest possible loss value, let us assume that each label $F_{y_i}$ is an independent variable. In OKO, we use a uniform sampler for the classes that are represented in $\gS = (\gS_x, \gS_y)$. Therefore, we spell out the OKO loss as 


\begin{align*}
    \gL (\theta) &= \frac{1}{N} \sum_{\gS_y } \sum_{\gS_x} \Pr[\gS_x | \gS_y] ( -\ve_1^\top \log(\softmax( f_\theta(\gS)))) \\
\end{align*}

where $\gS_y = \{ y_1', y_2',..., y_{k+2}'\}$ is the label set outputted by our sampler and is summed over all choices of our labels (note this implicitly is uniform over all subsets with $k+1$ classes), the second sum is done over all sets and $\Pr[\gS_x | \gS_y]$ is the conditional probability that $\gS_x$ is chosen given that the represented class labels are $y_1', y_2',..., y_{k+2}'$, where $y_1' = y_2'$ is repeated and $N$ is the total number of choices of $\gS_y$ is the normalization constant. Since $N$ is uninteresting and does not affect the analysis, it will be dropped.

Let $s_i = 1 -\epsilon$ be the proportion of class $C_i$ have feature $x$ (and we let $s_{y_i}$ be the proportion of the class corresponding to label $y_i$. Note that the probability that all features are $x$ means that $\Pr[\gS_x = \{x, x, ..., x\} | C] = \prod_{i \in \gS_y} s_i = (1-\epsilon)^{k+2} = 1 - (k+2) \epsilon + O(\epsilon^2)$, which is the most probable set conditioned on $C$. Let $F_x = f_\theta(x)$ be the predicted label of $x$. Now, since we assumed that $\log(\softmax(f_\theta(\gS))) \leq B$ in our domain and only $O(\epsilon)$ of the probability mass is on the remaining sets $\gS_x \setminus\{x\}$, we can decompose $\gL(\theta) = \Pr[\gS_x = \{x, x, ..., x\} | C] \gL_x + O(B\epsilon)$, where $\gL_x$ is the loss on the singleton set, 

\begin{align*}
\gL_x(F_x) &\propto \sum_{i=1}^C \sum_{\gS_y: y_1' = i} \left(\prod_{y_j \in \gS_y} s_{y_j}\right) ( -\ve_i^\top \log(\softmax((k+2)F_x)))  \\
&\propto \sum_{i=1}^C s_i \sum_{\gS_y: y_1' = i} \left(\prod_{y_j \in \gS_y, y_j \neq y_1'} s_{y_j}\right) ( -\ve_i^\top \log(\softmax((k+2)F_x)))  \\
&\propto \sum_{i=1}^C s_i \ve_i^\top \log(\softmax((k+2)F_x)) \\ 
\end{align*}

Note that an optimal solution of $\gL_x(F_x)$ is therefore $\softmax((k+2)F_x) \propto \, <s_1,..., s_m>$, where $m = C$ and the softmax is normalized to sum to 1, let us call such an optimal predicted label choice $F_x^\star$. By assumption, $s_i$ are equal, so in fact $H(\softmax(F_x)) = \log(|C|)$ has maximal entropy. %Furthermore, by our previous bounds, we see that $\gL(\theta^\star) \leq \gL(\theta) + O(B\epsilon)$. As before, we assume that the well-trained neural networks %Therefore, we conclude that for $\epsilon$ sufficiently small, we can show that by the local smoothness of $F$, $F_{\theta^\star}(x) = <s_1,..., s_m> + O(\epsilon)$, where the perturbation is bounded in $\epsilon$ element-wise. Since $s_i \approx 1$, we conclude that $H(F_{\theta^\star}(x)) = \log(|C|) - O(\epsilon)$.

Now, we show that for any $x' \in \gD', x' \neq x$, optimizing $F_{x'}$ in the OKO loss will also have high entropy even though the label is independent. To do this, we consider what we call the pair sets, which are sets with $\gS_{x_l} = \{x, ..., x, x_l\}$ with all features $x$ but only one data point in class $l$ that is not $x$. Note that $\Pr[\gS_x = \gS_{x_l} | C] = (1-s_l)\prod_{i \in \gS_y, i \neq l} s_i$. Therefore, since all $s_i = 1-\epsilon$, we may rewrite our total loss with the following decomposition of $\gL$: $\gL(\theta) = (1-\epsilon)^{k+2} \gL_x + \epsilon(1-\epsilon)^{k+1} \gL_{x'} + O(B\epsilon^2)$, where $\gL_{x'}$ is the loss on these pair sets: 

$$\gL_{x'}  = \sum_{i=1}^C s_i \sum_{\gS_y: y_1' = i} \sum_{y_l \in \gS_y} \left((1-s_{y_l}) \prod_{y_j \in \gS_y, y_j \neq y_l, y_1'} s_j \right) \sum_{x_l \in \gS_x: y = y_l} ( -\ve_i^\top \log(\softmax( (k+1)F_x + F_{x_l})))$$

where we sum over all possible choices of $y_l$ that is in $\gS_y$, which is the label of the pair class with non-shared feature $x_l \neq x$ and all choices of $x_l$ that has label $y_l$. 

Note that for each $x_l \neq x$, it is in exactly one pair set. For simplicity, let us consider $\gL_{x'}$ for a specific pair set and non-shared feature $x_l$ and we call the loss restricted to that set to be $\gL_{x_l}$. It suffices to show that a high entropy predictor minimizes $\gL_{x_l}$ and it will hold for the sum since each label $F_{x_l}$ is independent. Specifically, let $\Delta_l = F_{x_l} - F_x$, then we claim that $\Delta_l = 0$ minimizes $\gL_{x_l}$.

By isolating terms that depends on $\Delta_l$ and pulling out our label for $i$ and we can rewrite $\gL_{x_l}$ as a function of $\Delta_l$

$$ \gL_{x_l} = \sum_{i=1}^C -s_i e_i^\top \left(\sum_{\gS_y: y_1' = i, y_l \in \gS_y}  (1-s_l)\prod_{y_j \in \gS_y, y_j \neq y_l, y_1'} s_j  \log(\softmax((k+2) F_x + \Delta_l))  \right)$$

Now, since $1-s_i = \epsilon$ for all $i$, we may drop the terms depending on the product $s_i$ and we may rewrite as:

\begin{align*}
    \gL_{x_l} &\propto \sum_{i=1}^C -s_i e_i^\top \left( \sum_{\gS_y: y_1'=i, y_l \in \gS_y}  \log(\softmax((k+2)F_x + \Delta_l))  \right)\\
    &\propto \sum_{i=1}^C -s_i e_i^\top  \log(\softmax((k+2)F_x + \Delta_l)) \\
\end{align*}

where we exploited the uniformity of $\gS_y$. Now, we see that the minima of $\gL_{x_l}$ as a function of $\Delta_l$ therefore satisfies: $\softmax((k+2)F_x + \Delta_l) = < s_1,...,s_m>$, which means that $\Delta_l = 0$ minimizes $\gL_{x_l}$ and $H(\softmax(F_{x_l})) = \log(|C|)$ has maximal entropy. 

Therefore, we see that setting $\theta^\star$ such that $F_x = F_{x_l} = \alpha {\bf 1} $ is an exact loss minimizer of $\gL_x(F_x) + \sum_{x_l}(F_x, F_{x_l})$. From our decomposition of the total loss, since 

$\gL(\theta) = \gL_x(F_x) + \sum_{x_l} \gL_{x_l}(F_x, F_{x_l}) + O(B\epsilon^2)$

we conclude that $\gL(\theta^\star) \leq \min_{\theta} \gL(\theta) + O(B\epsilon^2)$.
\end{proof}

Note that the OKO loss on $\mathcal{D'}$ is quite small and relatively minimized at an excess loss of $O(\epsilon^2)$ even when the entropy of the prediction is high on the datapoints in $\mathcal{D}$. This is because the OKO loss implicitly averages the labels of all sets with datapoints in $\mathcal{D}$, which induces more entropy in the predictive distribution. As a point of comparison, for the cross entropy loss, such high prediction entropy everywhere will induce an excess loss of $O(\epsilon)$, as each datapoint in $\mathcal{D}$ will produce an excess loss of $\Omega(1)$ due to the uniform prediction, and these datapoints have mass $\Omega(\epsilon)$ in $\mathcal{D}'$ by construction.

